LAA-X: Unified Localized Artifact Attention for Quality-Agnostic and Generalizable Face Forgery Detection

In this paper, we propose Localized Artifact Attention X (LAA-X), a novel deepfake detection framework that is both robust to high-quality forgeries and capable of generalizing to unseen manipulations. Existing approaches typically rely on binary classifiers coupled with implicit attention mechanisms, which often fail to generalize beyond known manipulations. In contrast, LAA-X introduces an explicit attention strategy based on a multi-task learning framework combined with blending-based data synthesis. Auxiliary tasks are designed to guide the model toward localized, artifact-prone (i.e., vulnerable) regions. The proposed framework is compatible with both CNN and transformer backbones, resulting in two different versions, namely, LAA-Net and LAA-Former, respectively. Despite being trained only on real and pseudo-fake samples, LAA-X competes with state-of-the-art methods across multiple benchmarks. Code and pre-trained weights for LAA-Net\footnote{https://github.com/10Ring/LAA-Net} and LAA-Former\footnote{https://github.com/10Ring/LAA-Former} are publicly available.

==> tables/_cnn_vit_ssim_abl.tex <==
\begin{table*}
\centering
\caption{\textbf{Performance analyses across different levels of deepfake quality}. 
AUC (\%) comparisons between CNN-based methods (EFNB4~\cite{efn_net}+SBI~\cite{sbi}, Xception~\cite{xception}+SBI~\cite{sbi}, CADDM~\cite{caddm}, LAA-Net+SBI~\cite{laa_net}) and transformer-based methods (ViT~\cite{ViT}+SBI~\cite{sbi}, Swin~\cite{swin}+SBI~\cite{sbi}) across different deepfake quality levels assessed by the Mask SSIM~\cite{mssim_pose} metric.
The model is trained on FF++~\cite{ff++} and evaluated on CDF2~\cite{celeb_df}. 
}
\label{tabl:cnns_vit_ssim_abl}
\scalebox{1.0}{
% \resizebox{\textwidth}{!}{
\begin{tabular}{c| c|c|c|c|c|c}
\hline
\multirow{2}{*}{Method} & \multicolumn{6}{c}{Mask SSIM Ranges} \\
\cline{2-7}
 & $0.6$-$0.8$ $\uparrow$ & $0.8$-$0.9$ $\uparrow$ & $0.9$-$0.925$ $\uparrow$ & $0.925$-$0.95$ $\uparrow$ & $0.95$-$0.97$ $\uparrow$ & $0.97$-$1.0$ $\uparrow$ \\
 
\hline
\hline
ViT+SBI~\cite{sbi} & 90.5 & 94.0 & 89.2 & 84.7 & 82.1 & 78.0 \\
\cline{1-7}
EFNB4+SBI~\cite{sbi} & 89.3 & 84.1 & 80.3 & 83.6 & 82.8 & 78.6 \\
\cline{1-7}
Xception+SBI~\cite{sbi} & 82.9 & 80.6 & 80.5 & 85.0 & 82.3 & 79.4 \\
\cline{1-7}
CADDM~\cite{caddm} & 84.1 & 85.9 & 82.8 & 85.4 & 84.0 & 81.9 \\
\cline{1-7}
FA-ViT~\cite{FAViT} & - & - & - & - & - & - \\
\cline{1-7}
Swin+SBI~\cite{sbi} & 90.0 & 91.0 & 89.5 & 85.6 & 85.8 & 85.7 \\
\cline{1-7}
ForensicsAdapter~\cite{forensicsadapter} & - & - & - & - & - & - \\
\cline{1-7}
LAA-Net~\cite{laa_net} & 96.1 & 94.3 & 92.9 & 86.0 & 93.4 & 91.1 \\
\hline
\end{tabular}%
}
\end{table*}

